Sybil-Proof Diffusion Auction in Social Networks

A diffusion auction is a market to sell commodities over a social network, where the challenge is to incentivize existing buyers to invite their neighbors in the network to join the market. Existing mechanisms have been designed to solve the challenge in various settings, aiming at desirable properties such as non-deficiency, incentive compatibility and social welfare maximization. Since the mechanisms are employed in dynamic networks with ever-changing structures, buyers could easily generate fake nodes in the network to manipulate the mechanisms for their own benefits, which is commonly known as the Sybil attack. We observe that strategic agents may gain an unfair advantage in existing mechanisms through such attacks. To resist this potential attack, we propose two diffusion auction mechanisms, the Sybil tax mechanism (STM) and the Sybil cluster mechanism (SCM), to achieve both Sybil-proofness and incentive compatibility in the single-item setting. Our proposal provides the first mechanisms to protect the interests of buyers against Sybil attacks with a mild sacrifice of social welfare and revenue.

==> section/2_preliminaries/22_existing.tex <==


\subsection{Incentive Compatible Diffusion Auction Mechanisms}\label{h2:vcg-idm}

Various mechanisms have been proposed \cite{li:IDM} to achieve the aforementioned incentive compatibility goal. In this section, we will provide three examples.

The most trivial way to achieve IC in diffusion auctions is to ignore diffusion completely, treat it as a single-item auction, and perform a second-price auction on the seller's neighbors \(n(s)\). We will use \(\maxbid{S}\) to denote the highest bid in a set \(S\), or \(\maxbid{S}=\max_{x\in S} v'_x\).

\begin{definition}[NSP]\label{mechanism:NSP}
  The \emph{Neighbor Second-Price} (NSP) Auction is a mechanism that the item is sold to the highest bidder among the seller's neighbor \(x^*=\arg\max_{x\in n(s)}{v'_x}\). The winner pays to the seller the second highest bid in \(n(s)\), i.e. \(t_{x^*}=-\maxbid{n(s)\setminus\{x^*\}}\), and \(t_{s}=-t_{x^*}\).
\end{definition}

However, this trivial mechanism defeats the purpose of diffusion auctions, i.e., to utilize the social network structure to advertise the auction to a broader audience. To fulfill this goal while still respecting incentive compatibility, we can apply the famous VCG mechanism\cite{AGTbook2007} to our scenario. Recall that in VCG auction, each agent pays an amount equal to the social cost of their participation. In our scenario, an agent's diffusion may introduce new agents to the auction. Therefore, these agents' participation may increase the social welfare, instead of incurring a social cost, and should be rewarded by the auction.

\begin{framed}
 \label{mechanism:VCG}
 \noindent\textbf{VCG Mechanism}\\
 \rule{\textwidth}{0.5pt}

\begin{enumerate}
    \item Given the reported type profile \(\maskprofile\), we can find the highest bidder among the visible agents \(x^*=\arg\min_{x\in V(H)}{v'_x}\). This agent wins the item. Formally\footnotemark{}, \(\pi_{x^*}=1\). She also pays the second-highest price among all visible agents \(t_{x^*}=-\maxbid{V(H)\setminus \{x^*\}}\).
    \item Let \(\alpha(x)\) be the set of vertices \(y\) that, if \(x\) were not present, will not be reachable from the seller \(s\). The payment function of buyer \(x\neq x^*\) is \(t_x=\maxbid{V(H)}-\maxbid{V(H)\setminus \alpha(x)}\). Note that this value is equal to the increase in the social welfare due to the participation of \(x\).
    \item The allocation function and monetary transfer for other buyers are zero. The monetary transfer of seller is determined by the budget balance condition, i.e. \(t_s = -\sum_{x\neq s}{t_x}\).
\end{enumerate}
\end{framed}

\footnotetext{We omit the argument \((\maskprofile)\) in \(\pi_i(\maskprofile)\) and \(t_i(\maskprofile)\) when presenting mechanisms for better readability.}

In \cite{li:IDM}, Li et al. observed that VCG mechanism is IC and has optimal social welfare, but may have a budget deficit, i.e., the seller may have a negative profit because of the payments made to each intermediate buyers. They proposed Information Diffusion Mechanism (IDM) to tackle with this problem. 

We can observe that, in VCG, if an agent \(x\) receives a participation reward, she must be \emph{critical} for the diffusion to \(x^*\): Since \(x^*\in \alpha(x)\), \(s\) cannot reach \(x^*\) without the participation of \(x\). In graph theoretical terms\cite{lengauer:dominators}, this means that \(x\) dominates \(y\), and it is denoted as \(x \dom y\). We assert that \(x \dom x\) for every vertex \(x\). If \(x \dom y\), we say that \(x\) is a dominator of \(y\). The domination relationship is a partial order, and we can see that \(\alpha(x)=\left\{y\mid x\dom y\right\}\).

An \emph{immediate dominator} of \(x\), denoted as \(v=idom(x)\), is defined as the unique vertex \(v\) that dominates \(x\), and is dominated by every dominator \(w\neq v\) of \(x\). 

\begin{theorem}\label{thm:dom-tree}
Every vertex on the graph \(H\) except \(s\) has a unique immediate dominator, and \(\{(idom(x),x)\mid x\in V_{-s}\}\) forms a directed tree with \(s\) being its root, called the \emph{dominator tree} of \(H\) rooted at \(s\).
\end{theorem}

\begin{remark}
This is exactly Theorem 1 of \cite{lengauer:dominators}. The definition of dominators is identical to \emph{diffusion critical nodes} in \cite{li:IDM}, and the path from \(s\) to \(x\) on the dominator tree is the \emph{diffusion critical sequence} of \(x\), denoted as \(C_x\).
\end{remark}

\begin{framed}
 \label{mechanism:IDM}
 \noindent\textbf{Information Diffusion Mechanism (IDM)}\\
 \rule{\textwidth}{0.5pt}

\begin{enumerate}

    \item \label{step:idm:1} Given the reported type profile \(\maskprofile\), we can find the visible buyer with the highest bid, denoted by \(x^*\), where \(v'_{x^*}=\maxbid{V(H)}\).
    
    \item \label{step:idm:2} Compute the dominator sequence \(C_{x^*}=\{c_0=s,c_1,\dots,c_\ell=x^*\}\). Specifically, we have \(c_j = idom(c_{j+1})\), for all \(0 \le j < \ell\).

    \item \label{step:idm:3} We define \(p_j\) as the optimal social welfare when \(c_j\) is not present, and \(q_j\) as the optimal social welfare when all agents further in the \(C_{x^*}\) sequence are not present.
\begin{align*}
    p_j &= \maxbid{V(H)\setminus \alpha(c_j)},\\
    q_j &= \left\{
            \begin{aligned}
            &p_{j+1}       & \text{for }j < \ell,\\
            &\maxbid{V(H)} & \text{for } j = \ell.
            \end{aligned}
        \right.
\end{align*}
    \item \label{step:idm:4} Pick a \(c_d\) satisfying \(v'_{c_d}\geq q_d\); when there are multiple candidates, pick the one with the lowest index \(d\). Since \(q_\ell=\maxbid{V(H)}=v'_{c_\ell}\), such \(c_d\) must exist. This agent wins the item with \(\pi_{c_d}=1\).
    \item \label{step:idm:5} The payment of \(c_j\) is calculated as follows.
\[
t_{c_j}(\vek\theta')=\left\{
\begin{aligned}
q_j &{} - p_j &\text{for } & 1 \le j < d,\\
    &{} - p_j &\text{for } & j = d.
\end{aligned}
\right.
\]

\item \label{step:idm:6} The monetary transfer and allocation of all other buyers are zero. The revenue of the seller is \(t_s(\vek\theta')=-\sum_{1\leq j\leq d}{t_{c_j}}\).
\end{enumerate}
\end{framed}

It is proven in \cite{li:IDM} that IDM is IC, IR and non-deficit.

==> section/star-spdm.tex <==
Let \(\Gamma=\mpc(\Gamma_H\cup \Gamma')\) as defined in the previous section. It must be guaranteed that each vertex in \(\Gamma'\) must not be a false identity. We define \(\alpha(x)=\{y\mid x\dom y\},\oalpha(x)=\alpha(x)\setminus\{x\}\) and \(\gamma(x)=\bigcup_{y\in \Gamma\cap \oalpha(x)}{\alpha(y)}\). Intuitively, the set \(\oalpha(x)\) represents the possible Sybil identities of \(x\) without prior information, and \(\gamma(x)\) are the subset of \(\alpha(x)\) that must not be a Sybil identity of \(x\) with \(\Gamma\) given. We also define \(A(x)=V(H)\setminus \alpha(x)\).

For simplicity reasons, we will use \(\maxbid{S}\) to be the highest bid in a set \(S\), or \(\maxbid{S}=\max_{x\in S} b_x\). With these notations, we define our framework for Sybil proof diffusion mechanisms.

\subsection{{\STMfull}}

\input{section/mechanisms/deterministic}

\subsection{\SCMfull}\label{h2:scm}

\input{section/mechanisms/probabilistic}

